Linearly Convergent Frank-Wolfe with Backtracking Line-Search

Structured constraints in Machine Learning have recently brought the Frank-Wolfe (FW) family of algorithms back in the spotlight. While the classical FW algorithm has poor local convergence properties, the Away-steps and Pairwise FW variants have emerged as improved variants with faster convergence. However, these improved variants suffer from two practical limitations: they require at each iteration to solve a 1-dimensional minimization problem to set the step-size and also require the Frank-Wolfe linear subproblems to be solved exactly. In this paper, we propose variants of Away-steps and Pairwise FW that lift both restrictions simultaneously. The proposed methods set the step-size based on a sufficient decrease condition, and do not require prior knowledge of the objective. Furthermore, they inherit all the favorable convergence properties of the exact line-search version, including linear convergence for strongly convex functions over polytopes. Benchmarks on different machine learning problems illustrate large performance gains of the proposed variants.

==> JMLR/defs.tex <==
\usepackage{nccmath} % mfrac
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks=true,
%     linkcolor=mydarkblue,
%     citecolor=mydarkblue,
%     filecolor=mydarkblue,
%     urlcolor=mydarkblue]{hyperref}
%
% \captionsetup{justification=raggedright}

\definecolor{myblue}{HTML}{D2E4FC}
\newcommand*\mybluebox[1]{%
\colorbox{myblue}{\hspace{1em}#1\hspace{1em}}}
\newcommand{\blue}{\color{blue}}
\newcommand{\bl}{\color{blue}}


\definecolor{mygreen}{HTML}{008000}
\newcommand*\mygreenbox[1]{%
\colorbox{mygreen}{\hspace{1em}#1\hspace{1em}}}
\newcommand{\green}{\color{green}}



\definecolor{myorange}{HTML}{FFC48C}
\newcommand*\myorangebox[1]{%
\colorbox{myorange}{\hspace{1em}#1\hspace{1em}}}
\definecolor{Gray}{gray}{0.92}


\renewcommand{\green}{\color{green}}
\newcommand{\red}{\color{red}}

\DeclareMathOperator*{\argmin}{\mathbf{arg\,min}}
\DeclareMathOperator*{\argmax}{\mathbf{arg\,max}}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\sri}{sri}
\DeclareMathOperator*{\clip}{clip}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\loss}{loss}
\DeclareMathOperator*{\diam}{diam}
\DeclareMathOperator*{\PWidth}{PWidth}
\DeclareMathOperator*{\mDW}{mDW}
\DeclareMathOperator*{\PdirW}{PdirW}
\DeclareMathOperator*{\radius}{radius}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\Fix}{{Fix}}
\DeclareMathOperator*{\reg}{reg}
\DeclareMathOperator*{\domain}{dom}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\thinprox}{prox}
\newcommand{\LMO}{\mathbf{{LMO}}}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\face}{faces}
\DeclareMathOperator*{\cone}{cone}
\DeclareMathOperator*{\lin}{lin}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\def\RR{{\mathbb R}}
\def\EE{{\mathbb E}}
\def\DD{{\boldsymbol{D}}}
\def\HH{{\mathcal{H}}}

% \def\prox{{\mathbf{prox}}}
% \def\eprox{{\emph{\text{prox}}}}
\def\rr{{\boldsymbol r}}
\def\ss{{\boldsymbol s}}
\def\xx{{\boldsymbol x}}
\def\yy{{\boldsymbol y}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\ss{{\boldsymbol s}}
\def\dd{{\boldsymbol d}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\CC{{\boldsymbol C}}
\def\TT{{\boldsymbol T}}
\def\MM{{\mathcal M}}
\def\AA{{\mathcal A}}
\def\BB{{\mathcal B}}
\def\SS{{\mathcal S}}
\newcommand{\Econd}{\mathbf{E}}
\renewcommand{\aa}{\boldsymbol{a}}


\def\bphi{{\boldsymbol \phi}}
\def\balpha{{\boldsymbol \alpha}}
\def\defas{\stackrel{\text{def}}{=}}

\newtheorem{assumption}{Assumption}
% \newtheorem{theorem}{Theorem}
% \newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{remark}{Remark}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{axiom}{Axiom}


\newtheorem{innercustomtheorem}{Theorem}
\newenvironment{customtheorem}[1]
  {\renewcommand\theinnercustomtheorem{#1}\innercustomtheorem}
  {\endinnercustomtheorem}


\newtheorem{innercustomcorollary}{Corollary}
\newenvironment{customcorollary}[1]
  {\renewcommand\theinnercustomcorollary{#1}\innercustomcorollary}
  {\endinnercustomcorollary}


  \newtheorem{innercustomlemma}{Lemma}
  \newenvironment{customlemma}[1]
    {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
    {\endinnercustomlemma}

\makeatletter
\newenvironment{subtheorem}[1]{%
  \def\subtheoremcounter{#1}%
  \refstepcounter{#1}%
  \protected@edef\theparentnumber{\csname the#1\endcsname}%
  \setcounter{parentnumber}{\value{#1}}%
  \setcounter{#1}{0}%
  \expandafter\def\csname the#1\endcsname{\theparentnumber.\Alph{#1}}%
  \ignorespaces
}{%
  \setcounter{\subtheoremcounter}{\value{parentnumber}}%
  \ignorespacesafterend
}
\makeatother
\newcounter{parentnumber}


==> optml/paper/defs.tex <==
\usepackage{nccmath} % mfrac
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks=true,
%     linkcolor=mydarkblue,
%     citecolor=mydarkblue,
%     filecolor=mydarkblue,
%     urlcolor=mydarkblue]{hyperref}
%
% \captionsetup{justification=raggedright}

\definecolor{myblue}{HTML}{D2E4FC}
\newcommand*\mybluebox[1]{%
\vspace{-.1em}
\colorbox{myblue}{
\hspace{.1em}#1\hspace{.1em}
}
\vspace{-.1em}
}
\newcommand{\blue}{\color{blue}}
\newcommand{\bl}{\color{blue}}


\definecolor{mygreen}{HTML}{008000}
\newcommand*\mygreenbox[1]{%
\colorbox{mygreen}{\hspace{1em}#1\hspace{1em}}}
\newcommand{\green}{\color{green}}



\definecolor{myorange}{HTML}{FFC48C}
\newcommand*\myorangebox[1]{%
\colorbox{myorange}{\hspace{1em}#1\hspace{1em}}}
\definecolor{Gray}{gray}{0.92}


\renewcommand{\green}{\color{green}}
\newcommand{\red}{\color{red}}

\DeclareMathOperator*{\argmin}{\mathbf{arg\,min}}
\DeclareMathOperator*{\argmax}{\mathbf{arg\,max}}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\sri}{sri}
\DeclareMathOperator*{\clip}{clip}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\loss}{loss}
\DeclareMathOperator*{\diam}{diam}
\DeclareMathOperator*{\PWidth}{PWidth}
\DeclareMathOperator*{\mDW}{mDW}
\DeclareMathOperator*{\PdirW}{PdirW}
\DeclareMathOperator*{\radius}{radius}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\Fix}{{Fix}}
\DeclareMathOperator*{\reg}{reg}
\DeclareMathOperator*{\domain}{dom}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\thinprox}{prox}
\newcommand{\LMO}{\mathbf{{LMO}}}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\face}{faces}
\DeclareMathOperator*{\cone}{cone}
\DeclareMathOperator*{\lin}{lin}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\def\RR{{\mathbb R}}
\def\EE{{\mathbb E}}
\def\DD{{\boldsymbol{D}}}
\def\HH{{\mathcal{H}}}

% \def\prox{{\mathbf{prox}}}
% \def\eprox{{\emph{\text{prox}}}}
\def\rr{{\boldsymbol r}}
\def\ss{{\boldsymbol s}}
\def\xx{{\boldsymbol x}}
\def\yy{{\boldsymbol y}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\ss{{\boldsymbol s}}
\def\dd{{\boldsymbol d}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\CC{{\boldsymbol C}}
\def\TT{{\boldsymbol T}}
\def\MM{{\mathcal M}}
\def\AA{{\mathcal A}}
\def\BB{{\mathcal B}}
\def\SS{{\mathcal S}}
\newcommand{\Econd}{\mathbf{E}}
\renewcommand{\aa}{\boldsymbol{a}}


\def\bphi{{\boldsymbol \phi}}
\def\balpha{{\boldsymbol \alpha}}
\def\defas{\stackrel{\text{def}}{=}}

\newtheorem{assumption}{Assumption}


\newtheorem{innercustomtheorem}{Theorem}
\newenvironment{customtheorem}[1]
  {\renewcommand\theinnercustomtheorem{#1}\innercustomtheorem}
  {\endinnercustomtheorem}


\newtheorem{innercustomcorollary}{Corollary}
\newenvironment{customcorollary}[1]
  {\renewcommand\theinnercustomcorollary{#1}\innercustomcorollary}
  {\endinnercustomcorollary}


  \newtheorem{innercustomlemma}{Lemma}
  \newenvironment{customlemma}[1]
    {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
    {\endinnercustomlemma}

\makeatletter
\newenvironment{subtheorem}[1]{%
  \def\subtheoremcounter{#1}%
  \refstepcounter{#1}%
  \protected@edef\theparentnumber{\csname the#1\endcsname}%
  \setcounter{parentnumber}{\value{#1}}%
  \setcounter{#1}{0}%
  \expandafter\def\csname the#1\endcsname{\theparentnumber.\Alph{#1}}%
  \ignorespaces
}{%
  \setcounter{\subtheoremcounter}{\value{parentnumber}}%
  \ignorespacesafterend
}
\makeatother
\newcounter{parentnumber}


==> optml/presentation/defs.tex <==

\usepackage{nccmath} % mfrac

\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
% \usepackage[colorlinks=true,
%     linkcolor=mydarkblue,
%     citecolor=mydarkblue,
%     filecolor=mydarkblue,
%     urlcolor=mydarkblue]{hyperref}
%
% \captionsetup{justification=raggedright}

\definecolor{myblue}{HTML}{D2E4FC}
\newcommand*\mybluebox[1]{%
\colorbox{myblue}{\hspace{1em}#1\hspace{1em}}}
\newcommand{\blue}{\color{blue}}


\definecolor{mygreen}{HTML}{008000}
\newcommand*\mygreenbox[1]{%
\colorbox{mygreen}{\hspace{1em}#1\hspace{1em}}}
% \newcommand{\green}{\color{green}}



\definecolor{myorange}{HTML}{FFC48C}
\newcommand*\myorangebox[1]{%
\colorbox{myorange}{\hspace{1em}#1\hspace{1em}}}
\definecolor{Gray}{gray}{0.92}


% \newcommand{\green}{\color{green}}
% \newcommand{\red}{\color{red}}

\DeclareMathOperator*{\argmin}{\mathbf{arg\,min}}
\DeclareMathOperator*{\argmax}{\mathbf{arg\,max}}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\sri}{sri}
\DeclareMathOperator*{\clip}{clip}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\loss}{loss}
\DeclareMathOperator*{\diam}{diam}
\DeclareMathOperator*{\PWidth}{PWidth}
\DeclareMathOperator*{\mDW}{mDW}
\DeclareMathOperator*{\PdirW}{PdirW}
\DeclareMathOperator*{\radius}{radius}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\Fix}{{Fix}}
\DeclareMathOperator*{\reg}{reg}
\DeclareMathOperator*{\domain}{dom}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\thinprox}{prox}
\DeclareMathOperator*{\LMO}{\mathbf{{LMO}}}
\DeclareMathOperator*{\conv}{conv}
\DeclareMathOperator*{\face}{faces}
\DeclareMathOperator*{\cone}{cone}
\DeclareMathOperator*{\lin}{lin}

\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\def\RR{{\mathbb R}}
\def\EE{{\mathbb E}}
\def\DD{{\boldsymbol{D}}}
\def\HH{{\mathcal{H}}}

% \def\prox{{\mathbf{prox}}}
% \def\eprox{{\emph{\text{prox}}}}
\def\rr{{\boldsymbol r}}
\def\ss{{\boldsymbol s}}
\def\xx{{\boldsymbol x}}
\def\yy{{\boldsymbol y}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\ss{{\boldsymbol s}}
\def\dd{{\boldsymbol d}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\CC{{\boldsymbol C}}
\def\TT{{\boldsymbol T}}
\def\MM{{\mathcal M}}
\def\AA{{\mathcal A}}
\def\SS{{\mathcal S}}
\newcommand{\Econd}{\mathbf{E}}
\renewcommand{\aa}{\boldsymbol{a}}


\def\bphi{{\boldsymbol \phi}}
\def\balpha{{\boldsymbol \alpha}}
\def\defas{\stackrel{\text{def}}{=}}

% \newtheorem{assumption}{Assumption}
% \newtheorem{theorem}{Theorem}
% % \newtheorem{definition}{Definition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{remark}{Remark}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{axiom}{Axiom}
% 
% 
% \newtheorem{innercustomtheorem}{Theorem}
% \newenvironment{customtheorem}[1]
%   {\renewcommand\theinnercustomtheorem{#1}\innercustomtheorem}
%   {\endinnercustomtheorem}
% 
% 
% \newtheorem{innercustomcorollary}{Corollary}
% \newenvironment{customcorollary}[1]
%   {\renewcommand\theinnercustomcorollary{#1}\innercustomcorollary}
%   {\endinnercustomcorollary}
% 
% 
%   \newtheorem{innercustomlemma}{Lemma}
%   \newenvironment{customlemma}[1]
%     {\renewcommand\theinnercustomlemma{#1}\innercustomlemma}
%     {\endinnercustomlemma}

